Multimodal Data Visualization and Denoising with Integrated Diffusion

We propose a method called integrated diffusion for combining multimodal datasets, or data gathered via several different measurements on the same system, to create a joint data diffusion operator. As real world data suffers from both local and global noise, we introduce mechanisms to optimally calculate a diffusion operator that reflects the combined information from both modalities. We show the utility of this joint operator in data denoising, visualization and clustering, performing better than other methods to integrate and analyze multimodal data. We apply our method to multi-omic data generated from blood cells, measuring both gene expression and chromatin accessibility. Our approach better visualizes the geometry of the joint data, captures known cross-modality associations and identifies known cellular populations. More generally, integrated diffusion is broadly applicable to multimodal datasets generated in many medical and biological systems.

==> zzz_old.tex <==
\vskip -0.1in
\begin{algorithm}
  \caption{Local Denoising Procedure}
    \begin{algorithmic}[1]
    \REQUIRE Data set  $\mathbf{X}$ consisting of $\mathit{n}$ points obtained via a single measurement modality
    \ENSURE Locally denoised $\mathbf{X}$ 
    %%%
    \STATE Compute the affinity matrices on $\mathbf{X}$ as per Eq. (1)
    \STATE Partition the datasets into $\mathit{N}$ neighborhoods via spectral clustering 
    \STATE For every partition, $k_{1}, \ldots ,k_{N}$, compute PCA via singular value decomposition (SVD) of the neighborhood
    \STATE Estimate local intrinsic dimensionality using eigengap heuristic on singular values
    \STATE Compute a low-rank approximation of the SVD matrix to reconstruct a denoised set of data
  \end{algorithmic}
\end{algorithm}
\vskip -0.1in
